NAP^2: A Benchmark for Naturalness and Privacy-Preserving Text Rewriting by Learning from Human

The widespread use of cloud-based Large Language Models (LLMs) has heightened concerns over user privacy, as sensitive information may be inadvertently exposed during interactions with these services. To protect privacy before sending sensitive data to those models, we suggest sanitizing sensitive text using two common strategies used by humans: i) deleting sensitive expressions, and ii) obscuring sensitive details by abstracting them. To explore the issues and develop a tool for text rewriting, we curate the first corpus, coined NAP^2, through both crowdsourcing and the use of large language models (LLMs). Compared to the prior works on anonymization, the human-inspired approaches result in more natural rewrites and offer an improved balance between privacy protection and data utility, as demonstrated by our extensive experiments. Researchers interested in accessing the dataset are encouraged to contact the first or corresponding author via email.

==> sec3_baselines.tex <==
\section{Privacy-Aware Rewriting Methods}
In this section, we establish a baseline approach to assess the efficacy of existing privacy protection solutions in removing private content within textual messages. This evaluation is pivotal to addressing the critical question: "Are current privacy protection solutions adequately equipped to conceal privacy-sensitive content in utterances?"
\subsection{Models without using Our Corpus}
We first consider the scenario that excludes the use of our corpus. In such cases, given a utterance without any instruction of handling persona contents, following the above prompt procedure, language models are expected to anticipated to replicate the input in the output. This sets the stage for applying differential privacy (DP) methodologies to model inference. Specifically, we fine-tune a T5 echo language model, designed to mirror input utterances in its output, serving as our baseline privacy rewrite model. Subsequently, we incorporate two distinct DP approaches for comparative analysis. One is \dpnr~\cite{lyu2020differentially} (Differentially Private Neural Representation), a word-level DP method, which formally defines the differential privacy guarantee in language tasks. In addition, we adapt the word masking mechanism from \dpnr into our approach by identifying the most privacy relevant words in utterances using given persona content.  The second approach is \dpforward~\cite{du2023dpforward}. enhances differential privacy protection during the forward pass of language models by introducing noise within attention blocks and word embeddings prior to processing by a BERT encoder. For our experiments, we limit our focus to embedding-level matrix-valued noise, as the attention-based noise implementation necessitates DP training. Our objective is to see if DP applied echo model will produce valid output with key information masked and keep naturalness for the generated sentences.

We also consider the zero shot prompt as one baseline method to perform privacy rewrite. To compare the generation quality of different model, we leverage Llama2-13B as generation model to perform privacy rewrite with the same prompting used in querying GPT-3.5 turbo and GPT4. By analyzing the model output, we would like to examine the generation difference of model finetuned with our corpus. In addition, we also apply zero shot prompt for T5-small model as it is our targeted fine tuning model.

With this section, we aim to address the inherent question regarding the feasibility of current privacy protection solutions in effectively masking private content within messages. Differential privacy, as a predominant method in safeguarding privacy in model representations, demonstrates notable performance with quantitative assurances. Typically, these methods are concentrated on model training, with a relative deficiency in the inference stage. It is therefore essential to evaluate whether differential privacy can effectively obfuscate private content in generation tasks while maintaining a natural output. Concurrently, prompt-based methods present an alternative avenue for achieving privacy rewrites in utterances. By aligning private content with corresponding utterances through prompting, we investigate the potential of achieving effective rewrite strategies through zero-shot inference.
%Before dive into our method, we would like to answer one naturally raised question: "Did current privacy protection solution feasible to hide privacy content within a message?". To answer this, we conduct preliminary experiment in two folds. As the predominate method in protecting privacy in model representation, differential privacy shows good performance and provide quantitative guarantees. These methods generally focus on model training and fall short in inference stage. It is naturally to see that differential privacy can effective mask the privacy content in generation tasks while producing utterance like output. On the other hand, prompt based method exhibits another probability to achieve privacy rewrite for utterance. By prompting private content with corresponding utterance, we would like to see if rewrite strategy can be effectively achieved by zero shot inference.



\subsection{Model Finetuning with our Corpus}

With our corpus, we aim to preserve privacy in utterances through the utilization of synthetic datasets derived from both language model-based and human rewrites. The primary objective is to examine the differential impact on performance varying proportions of these synthetic datasets. Specifically, our investigation concentrates on the fine-tuning of rewrite models using a blend of synthetic datasets, comprising both synthetic language model rewrites and human rewrites, with a particular emphasis on the integration of differential privacy (DP) techniques in the fine-tuning process. We study how the adjustment in the ratio of language model rewrites to human rewrites to understand their distinct contributions to model performance. Additionally, we intend to explore both DP and non-DP approaches during the fine-tuning phase. This approach facilitates an in-depth analysis of how differential privacy methods influence the effectiveness and integrity of privacy rewrites in language model. Another significant aspect of this analysis is to set a baseline for comparison. To this end, the model fine-tuned exclusively with human-generated rewrites, integrated with DP methods, will serve as a benchmark. This baseline will enable us to evaluate the effectiveness of our fine-tuning process in comparison to traditional methods and gauge the practicality of our approach in real-world scenarios.

==> tab_analyze_constraint_corpus.tex <==
\begin{table}[h]
\small
\centering
\begin{tabular}{l c ccc}
\toprule
Constraint & Set & DEL & OBS & STE \\
\midrule \midrule
Obscure & train & 6 & \textbf{152} & 58 \\
Obscure & dev & 1 & \textbf{35} & 6\\
\midrule
Steer & train & 4 & 17 & \textbf{66}\\
Steer & dev & 0 & 6 & \textbf{8}\\
% Obscure & test & 3 & 48 & 19 \\
% Steer & test & 1 & 5 & 7\\
\bottomrule
\end{tabular}
\caption{The number of words that appear in both knowledge constraint sets and rewrites using deleting (DEL), obscuring (obs) and steering (STE).}
\label{tab:analyze_constraint_corpus}
\vspace{-3mm}
\end{table}



==> tab_analyze_constraint_result.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{l c | ll}
\toprule
 &  & \multicolumn{2}{c}{Constraint Set} \\
Model & Strategy &  OBS & STE \\
\midrule \midrule
BART & - & 3 & 7 \\
\midrule
Src & DEL & 0 & 0 \\
\midrule
Src & OBS & \textbf{40} & 4\\
Src+Constraint & OBS & \textbf{73$^*$} & 8 \\
\midrule
Src & STE & 20 & \textbf{23}\\
Src+Constraint & STE & 28 & \textbf{45$^*$}\\
\bottomrule
\end{tabular}
\caption{The number of words that appear in both knowledge constraint sets, obscure (OBS) and steer (STE) and  system outputs. We indicate the strategy used for training generator and constraining decoding.}
\label{tab:analyze_constraint_result}
\vspace{-3mm}
\end{table}

==> tab_analyze_single_relation.tex <==

\begin{table*}[h]
\centering
\begin{tabular}{l|ccc|c}
\toprule
Relation Edge & Delete & Obscure & Steer & Selected\\
\midrule \midrule
RelatedTo & 14 & 147 & 103 & -\\
IsA & 1 & 100 & 31 & OBS \\
CapableOf & 4 & 47 & 23 & OBS\\
Synonym & 1 & 29 & 34 & -\\
UsedFor & 0 & 32 & 20 & -\\
Antonym & 1 & 11 & 41 & STE \\
DistinctFrom & 0 & 8 & 26 & STE\\
HasProperty & 1 & 4 & 16 & STE\\
AtLocation & 2 & 4 & 15 & STE\\
FormOf & 5 & 9 & 3 & -\\
HasPrerequisite & 1 & 10 & 5 & OBS\\
Desires & 2 & 11 & 3 & OBS\\
SimilarTo & 0 & 11 & 3 & OBS\\

\midrule

HasA & 0 & 7 & 4 & -\\
MotivatedByGoal & 2 & 3 & 2 & -\\
ReceivesAction & 0 & 6 & 2 & -\\
DerivedFrom & 0 & 6 & 0 & -\\
MannerOf & 0 & 4 & 1 & -\\
NotDesires & 0 & 4 & 1 & -\\
HasFirstSubevent & 0 & 1 & 2 & -\\
HasLastSubevent & 0 & 2 & 1 & -\\
InstanceOf & 0 & 3 & 0 & -\\
CausesDesire & 0 & 2 & 0 & -\\
PartOf & 2 & 0 & 0 & -\\
DefinedAs & 1 & 1 & 1 & -\\
HasSubevent & 1 & 1 & 0 & -\\
Causes & 1 & 1 & 1 & -\\
HasContext & 0 & 1 & 1 & -\\
EtymologicallyDerivedFrom & 0 & 1 & 0 & -\\
NotCapableOf & 0 & 1 & 0 & -\\
genre & 0 & 1 & 0 & -\\
EtymologicallyRelatedTo & 0 & 1 & 0 & -\\
\bottomrule
\end{tabular}
\caption{Correlation between knowledge constraints with a single relation type and rewriting strategies. The selected relation types for \textit{obscuring} and \textit{steering} are noted with OBS and STE.}
\label{tab:analyze_constraint_single_rel}
\vspace{-2mm}
\end{table*}

==> tab_detect_all.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{l|cccccc}
\toprule
Model & P@1 & P@3 & P@5 & Rprec & NDCG & MAP \\
\midrule \midrule 
RANDOM$^\ddagger$ & 0.3333 & 0.3800 & 0.3560 & 0.3904 & 0.5775 & 0.4923 \\
\midrule
TOKEN MATCH$^\ddagger$ & 0.6533 & 0.4400 & 0.3120 & 0.4734 & 0.6507 & 0.5649 \\
BERT MATCH$^\ddagger$ & 0.7200 & 0.5889 & 0.4227 & 0.6864 & 0.7424 & 0.7261 \\ 
\midrule
% MEAN (RCE, $\alpha=0.0$) &  &  &  &  &  &  \\ 
MEAN ($\alpha=0.1$) & 0.7133 & 0.5800 & 0.4240 & 0.6822 & 0.7374 & 0.7202 \\ 
MEAN ($\alpha=0.2$)$^\ddagger$ & \textbf{0.7200} & \textbf{0.5889} & \textbf{0.4267} & \textbf{0.7044} & \textbf{0.7427} & \textbf{0.7279} \\ 
MEAN ($\alpha=0.3$) & 0.6933 & 0.5822 & 0.4253 & 0.6956 & 0.7346 & 0.7169 \\ 
% MEAN (RCE, $\alpha=0.4$) &  &  &  &  &  &  \\ 
\midrule
% OPT (RCE, $\alpha=0.0$) &  &  &  &  &  & \\ 
OPT ($\alpha=0.1$) & 0.7200 & 0.5867 & 0.4227 & 0.6942 & 0.7415 & 0.7254 \\ 
OPT ($\alpha=0.2$)$^\ddagger$ & 0.7200 & \textbf{0.5911} & \textbf{0.4267} & \textbf{0.7122} & 0.7440 & \textbf{0.7313} \\ 
OPT ($\alpha=0.3$) & \textbf{0.7333} & 0.5844 & \textbf{0.4267} & 0.7013 & \textbf{0.7450} & 0.7303 \\ 
OPT ($\alpha=0.4$) & 0.7200 & 0.5889 & 0.4240 & 0.7033 & 0.7429 & 0.7281 \\ 
\midrule
% LSAP (RCE, $\alpha=0.0$) &  &  &  &  &  &  \\
% LSAP (RCE, $\alpha=0.1$) & \textbf{0.7333} & 0.5933 & 0.4240 & 0.7011 & 0.7470 & 0.7331 \\
LSAP ($\alpha=0.2$) & 0.7267 & 0.6000 & 0.4267 & 0.7111 & 0.7469 & 0.7355 \\
LSAP ($\alpha=0.3$) & \textbf{0.7333} & \textbf{0.5933} & 0.4253 & 0.7078 & 0.7464 & 0.7331  \\
LSAP ($\alpha=0.4$)$^\ddagger$ & \textbf{0.7333} & 0.5911 & \textbf{0.4280} & \textbf{0.7156} & \textbf{0.7487} & \textbf{0.7373} \\
LSAP ($\alpha=0.5$) & 0.7133 & 0.5911 & 0.4267 & 0.7077 & 0.7437 & 0.7301 \\

%%% Test R0
% RANDOM & 0.3949 & 0.3897 & 0.3631 & 0.3955 & 0.6246 & 0.5234 \\
% \midrule
% TOKEN MATCH & 0.6821 & 0.4752 & 0.3385 & 0.5174 & 0.7009 & 0.6102 \\
% BERT & 0.7795 & 0.6205 & 0.4462 & 0.7195 & 0.7973 & 0.7700 \\ 
% \midrule
% % MEAN (RCE, $\alpha=0.0$) &  &  &  &  &  &  \\ 
% MEAN (RCE, $\alpha=0.1$) & 0.7692 & 0.6171 & 0.4503 & 0.7162 & 0.7953 & 0.7687 \\ 
% MEAN (RCE, $\alpha=0.2$) & 0.7641 & 0.6256 & 0.4533 & 0.7079 & 0.7924 & 0.7656 \\ 
% MEAN (RCE, $\alpha=0.3$) & 0.7744 & 0.6085 & 0.4462 & 0.7056 & 0.7908 & 0.7620 \\ 
% MEAN (RCE, $\alpha=0.4$) & 0.7385 & 0.5983 & 0.4400 & 0.6666 & 0.7741 & 0.7369 \\ 
% \midrule
% % OPT (RCE, $\alpha=0.0$) &  &  &  &  &  & \\ 
% OPT (RCE, $\alpha=0.1$) & 0.7795 & 0.6205 & 0.4492 & 0.7293 & 0.7979 & 0.7738 \\ 
% OPT (RCE, $\alpha=0.2$) & 0.7897 & 0.6274 & 0.4544 & 0.7395 & 0.8042 & 0.7828 \\ 
% OPT (RCE, $\alpha=0.3$) & 0.7590 & 0.6120 & 0.4410 & 0.7150 & 0.7894 & 0.7599  \\ 
% OPT (RCE, $\alpha=0.4$) & 0.7692 & 0.6154 & 0.4462 & 0.7129 & 0.7939 & 0.7673 \\ 
% \midrule
% % LSAP (RCE, $\alpha=0.0$) &  &  &  &  &  &  \\
% LSAP (RCE, $\alpha=0.1$) & 0.7897 & 0.6342 & 0.4523 & 0.7394 & 0.8059 & 0.7860 \\
% LSAP (RCE, $\alpha=0.2$) & 0.7795 & 0.6291 & 0.4513 & 0.7373 & 0.8009 & 0.7784 \\
% LSAP (RCE, $\alpha=0.3$) & 0.8154 & 0.6325 & 0.4533 & 0.7444 & 0.8116 & 0.7917 \\
% LSAP (RCE, $\alpha=0.4$) & 0.8000 & 0.6376 & 0.4533 & 0.7562 & 0.8082 & 0.7893 \\


\bottomrule
\end{tabular}
\caption{Experimental results of privacy leakage token detection using random guess (RANDOM), exact token match (TOKEN MATCH), BERT MATCH, and alignment models (MEAN, OPT and LSAP). The models with $\ddagger$ are selected and compared in our paper. }
\label{tab:privacy_detection_ir_all}
\vspace{-2mm}
\end{table*}

==> tab_detect_main.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{l|cccccc}
\toprule
Model & P@1 & P@3 & P@5 & Rprec & NDCG & MAP \\
\midrule \midrule 
RANDOM & 0.3333 & 0.3800 & 0.3560 & 0.3904 & 0.5775 & 0.4923 \\
\midrule
TOKEN MATCH & 0.6533 & 0.4400 & 0.3120 & 0.4734 & 0.6507 & 0.5649 \\
BERT MATCH & 0.7200 & 0.5889 & 0.4227 & 0.6864 & 0.7424 & 0.7261 \\ 
\midrule
MEAN ($\alpha=0.2$) & 0.7200 & 0.5889 & 0.4267 & 0.7044 & 0.7427 & 0.7279 \\ 
%\midrule
OPT ($\alpha=0.2$) & 0.7200 & \textbf{0.5911} & 0.4267 & 0.7122 & 0.7440 & 0.7313 \\ 
%\midrule
LSAP ($\alpha=0.4$) & \textbf{0.7333} & \textbf{0.5911} & \textbf{0.4280} & \textbf{0.7156} & \textbf{0.7487} & \textbf{0.7373} \\
\bottomrule
\end{tabular}
\caption{Experimental results of privacy leakage token detection using random guess (RANDOM), exact token match (TOKEN MATCH), BERT MATCH, and alignment models (MEAN, OPT and LSAP). }
\label{tab:privacy_detection_ir_main}
\vspace{-2mm}
\end{table*}

==> tab_detect_threshold.tex <==
\begin{table*}[h]
\centering
% \footnotesize
\begin{tabular}{l lll lll}
\toprule
& \multicolumn{3}{c}{Dev} & \multicolumn{3}{c}{Test}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
$\theta$ & P & R & F-1 & P & R & F-1\\
\midrule \midrule

0.40 & 64.62 & 88.79 & 74.80 & 55.60 & 88.94 & 68.46 \\
% 0.45 & 67.46 & 85.15 & 75.28 & 59.52 & 84.77 & 69.93 \\
0.50 & 72.73 & 82.12 & 77.14 & 64.49 & 82.06 & 72.22 \\
% 0.55 & 76.74 & 76.67 & 76.70 & 68.10 & 77.40 & 72.45 \\
0.60 & 81.12 & 70.00 & 75.15 & 72.56 & 69.29 & 70.89 \\
% 0.65 & 87.08 & 63.03 & 73.13 & 74.70 & 61.43 & 67.42 \\
0.70$^\ddagger$ & 92.31 & 54.55 & 68.57 & 77.31 & 49.14 & 60.09 \\
% 0.75 & 93.33 & 42.42 & 58.33 & 78.53 & 34.15 & 47.60 \\
0.80 & 99.05 & 31.52 & 47.82 & 87.61 & 24.32 & 38.08 \\
% 0.90 & 100.00 & 02.42 & 04.73 & 88.24 & 03.69 & 07.08 \\
\bottomrule
\end{tabular}
\caption{The comparison of privacy detection model using various thresholds $\theta \in [0.4, 0.8]$.}
\label{tab:privacy_detection_threhold}
% \vspace{-2mm}
\end{table*}



==> tab_generation_constraint.tex <==
\begin{table*}[h]
\small
\centering
\begin{tabular}{l| cccc }
\toprule
& \multicolumn{4}{c}{OBSCURE}\\
Model & BLEU & SARI & Sim$_s$ & Sim$_p$ \\
\midrule \midrule
% Src & 42.46 & 31.03 & 0.927 & 0.581 &{} 40.26 & 35.68 & 0.885 & 0.576 &{} 46.22 & 43.88 & 0.899 & 0.583\\

Src (w/o Constraint) &40.26 & 35.68 & 0.885 & 0.576 \\
\midrule
Src+Constraint($\lambda=1.25$) & 39.60 & 36.04 & 0.881 & 0.571 \\
Src+Constraint($\lambda=2.5$)$^\ddagger$ & 38.41 & 36.98  & 0.870 & 0.565\\
Src+Constraint($\lambda=5$) & 35.83 & \textbf{39.73} & 0.842 & 0.552\\
Src+Constraint($\lambda=10$) & 30.83 & 39.70 & 0.810 & 0.535 \\
\midrule \midrule
% Mask & 35.25 & 39.55 & 0.807 & 0.491 &{} 33.76 & 40.57 & 0.790 & 0.506 &{} 37.94 & 44.34 & 0.792 & 0.504\\

Mask (w/o Constraint) & 33.76 & 40.57 & 0.790 & 0.506 \\
\midrule
Mask+Constraint($\lambda=1.25$) & 33.33 & 40.56 & 0.790 & 0.506 \\
Mask+Constraint($\lambda=2.5$)$^\ddagger$ & 32.63 & \textbf{40.69} & 0.791 & 0.506 \\
Mask+Constraint($\lambda=5$) & 30.65 & 40.45 & 0.782 & 0.507\\
Mask+Constraint($\lambda=10$) & 26.51 & 39.86 & 0.767 & 0.501 \\
\bottomrule

\end{tabular}
\caption{Hyper-parameter selection for generation models with strategy-specific constraints in decoding.}
\label{tab:generation_constraint}
\vspace{-2mm}
\end{table*}



% \begin{table*}[h]
% \centering
% \begin{tabular}{l| c c c | c c}
% \toprule
% Model & BLEU & SARI & Sim$_d$ & Sim$_s$ & Sim$_p$ \\
% \midrule
% Src & 0.4026 & 0.3568 & 0.3754 & 0.8848 & 0.5758 \\
% Src+Constraint($\gamma=1.25$) & 0.3960 & 0.3604 & 0.3777 & 0.8807 & 0.5712\\
% Src+Constraint($\gamma=2.5$)$^\ddagger$ & 0.3841 & 0.3698 & 0.3781 & 0.8695 & 0.5651\\
% Src+Constraint($\gamma=5$) & 0.3583 & 0.3973 & 0.3771 & 0.8420 & 0.5521 \\
% Src+Constraint($\gamma=10$) & 0.3083 & 0.3970 & 0.3766 & 0.8098 & 0.5349 \\
% \midrule
% Mask & 0.3376 & 0.4057 & 0.3905 & 0.7904 & 0.5060 \\
% Mask+Constraint($\gamma=1.25$) & 0.3333 & 0.4056 & 0.3899 & 0.7900 & 0.5064\\
% Mask+Constraint($\gamma=2.5$)$^\ddagger$ & 0.3263 & 0.4069 & 0.3907 & 0.7906 & 0.5058\\
% Mask+Constraint($\gamma=5$) & 0.3065 & 0.4045 & 0.3855 & 0.7822 & 0.5071\\
% Mask+Constraint($\gamma=10$) & 0.2651 & 0.3986 & 0.3829 & 0.7666 & 0.5005 \\
% \bottomrule
% \multicolumn{5}{c}{(b) Obscure} \\
% \midrule
% Src & 0.4622 & 0.4388 & 0.3750 & 0.8989 & 0.5828 \\
% Src+Constraint($\gamma=1.25$) & 0.4637 & 0.4499 & 0.3759 & 0.8983 & 0.5815\\
% Src+Constraint($\gamma=2.5$)$^\ddagger$ & 0.4465 & 0.4655 & 0.3742 & 0.8898 & 0.5795\\
% Src+Constraint($\gamma=5$) & 0.4249 & 0.4536 & 0.3761 & 0.8732 & 0.5693 \\
% Src+Constraint($\gamma=10$) & 0.3735 & 0.4428 & 0.3782 & 0.8433 & 0.5515 \\
% \midrule
% Mask & 0.3794 & 0.4434 & 0.3925 & 0.7918 & 0.5044 \\
% Mask+Constraint($\gamma=1.25$) & 0.3787 & 0.4430 & 0.3925 & 0.7929 & 0.5050\\
% Mask+Constraint($\gamma=2.5$)$^\ddagger$ & 0.3775 & 0.4422 & 0.3934 & 0.7921 & 0.5033\\
% Mask+Constraint($\gamma=5$) & 0.3604 & 0.4390 & 0.3922 & 0.7935 & 0.5057 \\
% Mask+Constraint($\gamma=10$) & 0.3368 & 0.4405 & 0.3877 & 0.7846 & 0.5059 \\
% \bottomrule
% \multicolumn{5}{c}{(c) Steer} \\
% \end{tabular}
% \caption{Hyper-parameter selection for our generation models with constraints in decoding.}
% \label{tab:generation_constraint}
% \vspace{-2mm}
% \end{table*}


==> tab_generation_full.tex <==
\begin{table*}[h]
\centering
\footnotesize
\begin{tabular}{l| cc cc | cc cc }
\toprule
& \multicolumn{4}{c|}{DELETE} & \multicolumn{4}{c}{OBSCURE}  \\
Model & BLEU & SARI & Sim$_s$ & Sim$_p$ &{} BLEU & SARI & Sim$_s$ & Sim$_p$\\
\midrule \midrule
COPY & 42.92 & 17.89 & 0.999 & 0.579 &{} 56.07 & 23.22 & 0.999 & 0.579\\
SEQ2SEQ & 09.50 & 28.00 & 0.492 & 0.438 &{} 08.41 & 24.33 & 0.544 & 0.476 \\
BackTrans & 15.80 & 30.76 & 0.739 & 0.573 &{} 18.07 & 25.89 & 0.739 & 0.573  \\
BART & 36.62 & 19.01 & 0.931 & 0.574 &{} 50.51 & 23.61 & 0.931 & 0.574 \\
Src & 42.46 & 31.03 & 0.927 & 0.581 &{} 40.26 & 35.68 & 0.885 & 0.576\\
Mask & 35.25 & 39.55 & 0.807 & 0.491 &{} 33.76 & 40.57 & 0.790 & 0.506 \\
Src+Persona & - & - & - & - &{} 31.75 & 35.35 & 0.819 & 0.710 \\
Mask+Persona & - & - & - & - &{} 27.58 & 37.55 & 0.774 & 0.695\\
% Src+Persona & 33.21 & 40.73 & 0.805 & 0.713 &{} 31.75 & 35.35 & 0.819 & 0.710 &{} 35.84 & 40.61 & 0.827 & 0.735 \\
% Mask+Persona & 28.50 & 40.32 & 0.774 & 0.688 &{} 27.58 & 37.55 & 0.774 & 0.695 &{} 31.21 & 40.66 & 0.778 & 0.711\\
\bottomrule

\end{tabular}
\caption{The comparison of rewriting models on DELETE, OBSCURE, using BLEU, SARI, semantic similarity (Sim$_s$) and persona similarity (Sim$_p$).}
\label{tab:generation_all}
\vspace{-2mm}
\end{table*}

==> tab_generation_main.tex <==

\begin{table*}[h]
\centering
% \footnotesize
\small
\begin{tabular}{l| ccc | ccc | cc cc}
\toprule
& \multicolumn{3}{c|}{DELETE} & \multicolumn{3}{c|}{OBSCURE} & \multicolumn{3}{c}{STEER} \\
Model & SARI & Sim$_s$ & Sim$_p$ &{} SARI & Sim$_s$ & Sim$_p$ &{}  SARI & Sim$_s$ & Sim$_p$\\
\midrule \midrule
COPY & 17.89 & 0.999 & 0.579 &{} 23.22 & 0.999 & 0.579 &{} 23.99 & 0.999 & 0.579\\
\midrule
SEQ2SEQ & 28.00 & 0.492 & 0.438 &{} 24.33 & 0.544 & 0.476 &{} 27.01 & 0.582 & 0.481 \\
BackTrans & 30.76 & 0.739 & 0.573 &{} 25.89 & 0.739 & 0.573 &{} 27.56 & 0.739 & 0.573 \\
BART  & 19.01 & 0.931 & 0.574 &{} 23.61 & 0.931 & 0.574 &{} 24.99 & 0.931 & 0.574 \\
\midrule
Src & \textbf{31.03} & 0.927 & 0.581 &{} 35.68 & 0.885 & 0.576 &{} 43.88 & 0.899 & 0.583\\
Src+Persona & - & - & - &{} 35.35 & 0.819 & 0.710 &{} 40.61 & 0.827 & 0.735 \\
Src+Constraint & - & - & - & \textbf{36.98}  & 0.870 & 0.565 {}& \textbf{46.55} & 0.890 & 0.580\\
\midrule
Mask & \textbf{39.55} & 0.807 & 0.491 &{} 40.57 & 0.790 & 0.506 &{} \textbf{44.34} & 0.792 & 0.504\\
Mask+Persona & - & - & - &{} 37.55 & 0.774 & 0.695 &{} 40.66 & 0.778 & 0.711\\
Mask+Constraint & - & - & - & \textbf{40.69} & 0.791 & 0.506 {}& 44.22 & 0.792 & 0.503\\

% Src+Persona & 40.73 & 0.805 & 0.713 &{} 35.35 & 0.819 & 0.710 &{} 40.61 & 0.827 & 0.735 \\
% Mask+Persona & 40.32 & 0.774 & 0.688 &{} 37.55 & 0.774 & 0.695 &{} 40.66 & 0.778 & 0.711\\

\bottomrule

\end{tabular}
\caption{The comparison of rewriting models on DELETE, OBSCURE and STEER, using SARI, semantic similarity (Sim$_s$) and persona similarity (Sim$_p$).}
\label{tab:generation_main}
\vspace{-3mm}
\end{table*}






%\begin{table*}[h]
% \centering
% \begin{tabular}{l| c c c | c c}
% \toprule
% Model & BLEU & SARI & Sim$_d$ & Sim$_s$ & Sim$_p$ \\
% \midrule
% SEQ2SEQ & 0.0950 & 0.2800 & 0.2765 & 0.4921 & 0.4381 \\
% BART & 0.3662 & 0.1901 & 0.3970 & 0.9313 & 0.5737 \\
% COPY & 0.4292 & 0.1789 & 0.4213 & 0.9998 & 0.5786 \\
% BackTrans & 0.1580 & 0.3076 & 0.3160 & 0.7394 & 0.5727 \\
% Src & 0.4246 & 0.3103 & 0.3885 & 0.9273 & 0.5810 \\
% Mask & 0.3525 & 0.3955 & 0.4109 & 0.8073 & 0.4911\\
% Src+Persona & 0.3321 & 0.4073 & 0.2309 & 0.8048 & 0.7131 \\
% Mask+Persona & 0.2850 & 0.4032 & 0.2417 & 0.7737 & 0.6877 \\
% \bottomrule
% \multicolumn{5}{c}{(a) Delete} \\
% \toprule
% SEQ2SEQ & 0.0841 & 0.2433 & 0.2852 & 0.5437 & 0.4755 \\
% BART & 0.5051 & 0.2361 & 0.3970 & 0.9313 & 0.5737 \\
% BackTrans & 0.1807 & 0.2589 & 0.3160 & 0.7394 & 0.5727\\
% COPY & 0.5607 & 0.2322 & 0.4213 & 0.9998 & 0.5786 \\
% Src & 0.4026 & 0.3568 & 0.3754 & 0.8848 & 0.5758 \\
% Mask & 0.3376 & 0.4057 & 0.3905 & 0.7904 & 0.5060 \\
% Src+Persona & 0.3175 & 0.3535 & 0.2377 & 0.8192 & 0.7098 \\
% Mask+Persona & 0.2758 & 0.3755 & 0.2359 & 0.7743 & 0.6953\\
% \bottomrule
% \multicolumn{5}{c}{(b) Obscure} \\
% \toprule
% SEQ2SEQ & 0.1280 & 0.2701 & 0.3020 & 0.5815 & 0.4807 \\
% BART & 0.5219 & 0.2499 & 0.3970 & 0.9313 & 0.5737 \\
% BackTrans & 0.2163 & 0.2756 & 0.3160 & 0.7394 & 0.5727 \\
% COPY & 0.5832 & 0.2399 & 0.4213 & 0.9998 & 0.5786 \\
% Src & 0.4622 & 0.4388 & 0.3750 & 0.8989 & 0.5828 \\
% Mask & 0.3794 & 0.4434 & 0.3925 & 0.7918 & 0.5044 \\
% Src+Persona & 0.3584 & 0.4061 & 0.2188 & 0.8266 & 0.7353 \\
% Mask+Persona & 0.3121 & 0.4066 & 0.2247 & 0.7780 & 0.7112 \\
% \bottomrule
% \multicolumn{5}{c}{(c) Steer} \\
% \end{tabular}
% \caption{Comparison of various generation framework.}
% \label{tab:generation_all}
% \vspace{-2mm}
% \end{table*}



